Software for the SpaceDREAM Robotic Arm

Impedance-controlled robots are widely used on Earth to perform interaction-rich tasks and will be a key enabler for In-Space Servicing, Assembly and Manufacturing (ISAM) activities. This paper introduces the software architecture used on the On-Board Computer (OBC) for the planned SpaceDREAM mission aiming to validate such robotic arm in Lower Earth Orbit (LEO) conducted by the German Aerospace Center (DLR) in cooperation with KINETIK Space GmbH and the Technical University of Munich (TUM). During the mission several free motion as well as contact tasks are to be performed in order to verify proper functionality of the robot in position and impedance control on joint level as well as in cartesian control. The tasks are selected to be representative for subsequent servicing missions e.g. requiring interface docking or precise manipulation. The software on the OBC commands the robot's joints via SpaceWire to perform those mission tasks, reads camera images and data from additional sensors and sends telemetry data through an Ethernet link via the spacecraft down to Earth. It is set up to execute a predefined mission after receiving a start signal from the spacecraft while it should be extendable to receive commands from Earth for later missions. Core design principle was to reuse as much existing software and to stay as close as possible to existing robot software stacks at DLR. This allowed for a quick full operational start of the robot arm compared to a custom development of all robot software, a lower entry barrier for software developers as well as a reuse of existing libraries. While not every line of code can be tested with this design, most of the software has already proven its functionality through daily execution on multiple robot systems.

==> images-src/makefile <==
# Makefile under working under windows using:
# Inkscape 1.1.1
# mingw32-make (if you have R installed, it should be available here: C:/Users/YOUR_USERNAME/Documents/R/win-library/3.6/Rtools/mingw_64/bin/

# This is where the exported 'compiled' images will be written to.
BIN_DIR = ../images-bin

# Number of columns in the paper. Used to determine appropriate bitmap width.
N_COLUMNS = 2
# Resolution of bitmaps. Used to determine appropriate bitmap width.
#   standard: resolution for screen, usually fine for camera-ready also (default)
#   high: resolution for printing (official recommendation for line art by IEEE)
RESOLUTION = standard

################################################################################
# GATHER RELEVANT SOURCES AND DETERMINE TARGETS

SOURCES_SVG := $(shell find ./ -name "*.svg")
# Standard: convert SVG to PDF and include it in the TEX file.
TARGETS += $(subst .svg,-svg.pdf,${SOURCES_SVG})
# If the PDF is too large for some reason (1000s data points), include the PNG in the TEX instead. 
TARGETS += $(subst .svg,-svg-png.png,${SOURCES_SVG})
# Worst possible idea to convert SVG to JPG. But some journals want JPG.
# TARGETS += $(subst .svg,-svg-jpg.jpg,${SOURCES_SVG})

SOURCES_FIG := $(shell find ./ -maxdepth 1 -name '*.fig')
TARGETS += $(subst .fig,-fig.pdf,${SOURCES_FIG})

SOURCES_GIF := $(shell find ./ -maxdepth 1 -name '*.gif')
TARGETS += $(subst .gif,-gif.png,${SOURCES_GIF})

SOURCES_EPS := $(shell find ./ -maxdepth 1 -name '*.eps')
TARGETS += $(subst .eps,-eps.pdf,${SOURCES_EPS})

# Add output directory to the TARGETS
TARGETS := $(addprefix ${BIN_DIR}/,${TARGETS})


################################################################################
# TARGETS

all: ${BIN_DIR} ${TARGETS}

${BIN_DIR}:
	mkdir ${BIN_DIR}

clean:
	rm -f ${TARGETS}

clobber:
	rm -rf ${BIN_DIR}


################################################################################
# INKSCAPE EXPORT COMMANDS

INKSCAPE_VERSION:=$(shell python3 check_version.py)

ifeq (${INKSCAPE_VERSION}, 0)
	# Inkscape 0.x.x
	#   --without-gui         : Don't start inkscape GUI
	#   --export-area-drawing : Bounding box tight around the actual drawing
	#   --export-text-to-path : Convert text to paths before exporting
	SVG_EXPORT = inkscape --without-gui --export-area-drawing --file=$< 
	SVG_PDF_EXPORT = ${SVG_EXPORT} --export-text-to-path --export-pdf=$@
	SVG_BITMAP_EXPORT = ${SVG_EXPORT} --export-png=$@
else
	# Inkscape 1.x.x (default)
	#   --export-area-drawing : Bounding box tight around the actual drawing
	SVG_EXPORT = inkscape --export-area-drawing $< --export-filename=$@
	SVG_PDF_EXPORT = ${SVG_EXPORT}
	SVG_BITMAP_EXPORT = ${SVG_EXPORT}
endif

################################################################################
# APPROPRIATE WIDTH OF BITMAPS
#
# Determine appropriate width of bitmaps given one/two column and standard/high resolution.
# https://journals.ieeeauthorcenter.ieee.org/create-your-ieee-journal-article/create-graphics-for-your-article/resolution-and-size/
ifeq (${N_COLUMNS}, 1)
  # "\columnwidth with one column: 7.16 inches
  ifeq (${RESOLUTION}, high)
    BITMAP_WIDTH = 4296 # 7.16inch * 600dpi 
  else
    BITMAP_WIDTH = 2148 # 7.16inch * 300dpi 
  endif
else
  # "\columnwidth with two columns:  3.5 inches
  ifeq (${RESOLUTION}, high)
    BITMAP_WIDTH = 2100 # 3.5inch * 600dpi 
  else
    BITMAP_WIDTH = 1050 # 3.5inch * 300dpi 
  endif
endif

SVG_BITMAP_EXPORT += --export-width=${BITMAP_WIDTH}


################################################################################
# PATTERN RULES

# PDF from SVG
${BIN_DIR}/%-svg.pdf:%.svg
	@echo "$< -> $@"
	@${SVG_PDF_EXPORT} 2> /dev/null > /dev/null

# PNG from SVG
${BIN_DIR}/%-svg-png.png:%.svg
	@echo -n "$< -> $@" 
	@echo " (${N_COLUMNS}-column paper, ${RESOLUTION} resolution => bitmap width is ${BITMAP_WIDTH} pixels)"
	@${SVG_BITMAP_EXPORT} 2> /dev/null > /dev/null 

# JPG from PNG from SVG 
${BIN_DIR}/%-svg-jpg.jpg:${BIN_DIR}/%-svg-png.png
	@echo "$< -> $@"
	convert -background white -alpha remove -alpha off $< $@ 

# PDF from EPS
${BIN_DIR}/%-eps.pdf:%.eps ${BIN_DIR}
	@echo "$< -> $@"
	@epstopdf $< $@

# PNG from GIF: Only first frame [0] in case it is an animated gif.
${BIN_DIR}/%-gif.png:%.gif ${BIN_DIR}
	@echo "$< -> $@"
	@convert $<[0] $@
